Deconstructing Human-AI Collaboration: Agency, Interaction, and Adaptation

As full AI-based automation remains out of reach in most real-world applications, the focus has instead shifted to leveraging the strengths of both human and AI agents, creating effective collaborative systems. The rapid advances in this area have yielded increasingly more complex systems and frameworks, while the nuance of their characterization has gotten more vague. Similarly, the existing conceptual models no longer capture the elaborate processes of these systems nor describe the entire scope of their collaboration paradigms. In this paper, we propose a new unified set of dimensions through which to analyze and describe human-AI systems. Our conceptual model is centered around three high-level aspects - agency, interaction, and adaptation - and is developed through a multi-step process. Firstly, an initial design space is proposed by surveying the literature and consolidating existing definitions and conceptual frameworks. Secondly, this model is iteratively refined and validated by conducting semi-structured interviews with nine researchers in this field. Lastly, to illustrate the applicability of our design space, we utilize it to provide a structured description of selected human-AI systems.

==> cache.tex <==

\textbf{Motivational/Intro Sentence}

As complete AI-based automation remains out of reach in most real-world applications the focus has instead shifted to leveraging the strengths of both human and AI agents to create effective collaborative systems. Progress in this field has resulted in increasingly more complex/elaborate systems and frameworks while the language used to describe them has gotten more vague. Similarly the existing conceptual models no longer have enough breath to describe the entire scope of this (Human-AI) collaboration paradigm. 

joint-performance
\\ 

\textbf{What is this paper about?}

In this work, we propose a unified set of dimensions through which to model and describe human-AI collaborative systems and interactions. By deconstructing this multi-faceted collaboration from the perspectives of agency, interaction and adaptation we introduce a structured means to analyse?, compare and design human-AI systems 

Through our By deconstructing this multi-faceted collaboration from the perspectives of agency, interaction, and adaptation we introduce a structured means to analyze?, compare and design human-AI systems  
\\ 

\textbf{What's the major contribution? }

\begin{itemize}
    \item We propose a design space for human-AI collaboration
    
    \item Construct an initial prototype by surveying the literature and consolidating existing definitions and conceptual frameworks. 
    \item We iteratively refined and validated our conceptual model by conducting Semi-structured interviews with xy VA experts
    
    \item lastly, to illustrate the applicability of our design space, we utilize it to provide a structured description of selected human-AI systems
    
    our paper provides and exemplification of .. Exemplified application of this dimensionality 
\end{itemize}


A set of dimensions that effectively bridges the various components that make up human-AI collaboration like communication, interaction

Unify the community behind a single definition
\\ 

\textbf{What are the main steps of your approach?}

 extracted from existing literature
 
We survey literature consider existing definitions and their strengths and shortcomings to establish a minimum set of dimensions needed to effectively model any human-AI collaborative systems

Consolidated existing definitions and conceptual frameworks. 

A set of semi-structured interviews to iteratively improve and evaluate the proposed approach.

Application to 
\\ 

\textbf{How did you evaluate your approach?}

We encode some common systems without dimensionality.
\\ 

\textbf{What's the main result of the evaluation?}
That it works and makes sense?





